Language Models as Critical Thinking Tools: A Case Study of Philosophers

Current work in language models (LMs) helps us speed up or even skip thinking by accelerating and automating cognitive work. But can LMs help us with critical thinking -- thinking in deeper, more reflective ways which challenge assumptions, clarify ideas, and engineer new concepts? We treat philosophy as a case study in critical thinking, and interview 21 professional philosophers about how they engage in critical thinking and on their experiences with LMs. We find that philosophers do not find LMs to be useful because they lack a sense of selfhood (memory, beliefs, consistency) and initiative (curiosity, proactivity). We propose the selfhood-initiative model for critical thinking tools to characterize this gap. Using the model, we formulate three roles LMs could play as critical thinking tools: the Interlocutor, the Monitor, and the Respondent. We hope that our work inspires LM researchers to further develop LMs as critical thinking tools and philosophers and other 'critical thinkers' to imagine intellectually substantive uses of LMs.

==> draft-1.tex <==

\section{Introduction: The Horizon of Language Model Reasoning}

People have talked a lot about common-sense reasoning and more specialized reasoning, e.g. in the sciences or physically speaking.
What's interesting is that philosophy doesn't have to concern itself with the specialized domains per se, and it can even then talk about it; but it is concerned more or less with challenging or interrogating what is held as ``common sense'', or the tools which we use as common sense.

What is time?
What are alternative systems for establishing equality between people?
What kinds of evidence is acceptable to make judgements?

Researchers in language models (LMs) have made substantive advances in both the development and evaluation of sophisticated LM behavior.
For instance, there has been a lot of work on ethical reasoning, common-sense reasoning, etc.
Without being too idealist, one `ultimate' form of reasoning is philosophy.
Many of these developments are both near and far.

Some have even suggested that philosophy is the culmination of the human mind (hegel, decartes); others are more tame.

\textbf{Our main claim is that philosophy is an interesting and important `task' for LM researchers to think about}, because philosophy synthesizes and makes concrete many of the goals LM researchers want for LMs, but is also more accessible in the sense that philosophical notions and questions are embedded into every act; it is less restrictive, which is why proverbially for any $X$ there is a `philosophy of $X$.

Philosophical development is a great way to concretely represent these sorts of nuances in practice which we are concerned about when we talking about `reasoning'.
Yejin Choi says that commonsense reasoning is the dark matter of intelligence, and that may be so, but luckily one of the aims of philosophy as a field is to systematically work through the pitfalls and systems of reasoning.
It's very broad, lets you have your hands in many different places.

Methodologically, we conduct individual 30-60 minute interviews with \textbf{21 philosophy professors} from \textbf{14 philosophy departments} at research universities around the United States. % need to double check numbers
Further information about our interviewees is available in Table X.
We obtained a university IRB and received verbal consent from participants to participate in the study and to record.
We use the results to better inform and understand what they think about LMs, what they can imagine for LMs, and how philosophy can benefit the LM science.
In cases where philosophers knew little about LMs and hadn't interacted with them, we demoed with GPT-4 in an open-ended format.
Interview questions are included in the appendix.

\section{On `Doing' Philosophy}
In this section, we will present what philosophers described in the `doing' of philosophy.
We have two aims: to convince LM scientists that philosophy is an interesting and important “task” for understanding LM reasoning skills; and that  the best way to evaluate the “doing” of philosophy is to evaluate how well LMs can support philosophers in their work in philosophically substantive ways.

\subsection{Aims and intellectual movements}

\subsection{Material processes}
Interlocutors, etc.

\textbf{Conversation} has been a fundamental structure in philosophy, from Socrates in the Western tradition and even earlier in other traditions.
In fact, many participants mention that they 

\subsection{What makes philosophy difficult?}

\subsection{Can language models `do' philosophy?}

People have trained models on philosopher texts.
This may go far, but the success metric for language models doing philosophy shouldn't be the turing test, at least in any simple, experimental setting.

It should really be about how can language models support the doing of philosophy.


\section{Near and Far: Why LM researchers should care about philosophy}


\section{A Design Space for LMs `Doing' Philosophy}


\andre{everything below this line -- needs to be reworked and incorporated}


Currently: ChatGPT is selfless and controlled
Selfhood and controlled?
Selfhood and uncontrolled?
Selfless and uncontrolled?
These are all good 

In fact, this framework captures why existing language models tend to be uncompelling for philosophers.
In the process of doing philosophy, being in total control is difficult because you don't know where you're going. Add onto that a totally selfless mirror, and it's like what is going on.

A selfless and uncontrolled model can serve as a kind of tapestry for inspiration

Selfhood and uncontrolled is like reading a text -- how might that be valuable?

\textit{Selfhood} is the taking on of a particular perspective, having some semblance based on judgment, sort of self-ness; this does not mean dogmatic or unwilling to change views, but it does mean some kind of local consistency, judgment, bite.
Ian: an antagonistic AI, a critic AI.
Or just taking on various objective perspectives, even offensive ones, can be very useful.
Annette: if someone unsavory agrees with your view, that tells you something about how you've formulated it.

Selfhood and controlled is like a hostile commentator, someone who interacts and critiques with ideas (like a conversation)

These function along text vs. conversation.

In the matrix, we've put various roles and functions which we will elucidate more in the following section.
We find that philosophers' ideas about what will be useful are captured fairly well.

3 x 3 matrix: selfhood vs. control.
You can have a strong sense of selfhood against control.

\section{Opportunities and Challenges}
Discussion of the unique challenges of language models

\section{Recommendations}

\section{Conclusion}

Philosophy is interesting and important, because reasoning is so important in it... but it's also more.
The simultaneous tangability and challenge to NLP. Certainly, domain knowledge is important... but the focus is maybe less so on getting what others have said ``right'' in the same way that it might be in the natural sciences.

``
``Accuracy and factuality remain key concerns for using AI in the discovery process.''



















There are various roles that language models could play for philosophy which fall \textit{across} this matrix.
i.e., there are many different ways you could implement it.

\textit{Interlocutor.}
Principles of charity, understanding, exchanging ideas -- like one would with a real philosopher.
The benefit is that it might be able to provide many more perspectives.
Indeed, such an interlocutor could also take on various demeanors, including hostile or aggressive ones (Prasanta).
Requires high selfhood, various levels of control.

\textit{Questioner.}
If you have less control, your LM might be an effective questioner; it might ask effective questions to engage with.
But it could also sort of be selfless. The important thing is that it doesn't have control.
We emphasize this part: LMs don't really ask you questions, or if you do, the questions are fairly uninteresting and unhelpful.
In fact, there are a whole host of nuances that go into asking good questions. (Hannah)

\textit{Checks and balances.}
Ceding control. Self or not self.
Consciousness-raising, making things and decisions more present.
At various decision junctures, how can we be more conscious and not miss so many things?
Back to Decartes and doubt, in practice!
Metaphilosophical reconciler: the periphery and the canon.
We can link together the periphery and the canon in more compelling ways.

Broader significance to philosophy


==> junk.tex <==
% they might ask if a theory satisfies certain theoretical desiderata, and then ask how they set out normative desiderata to begin with.


% Using philosophy as a case study, we seek to investigate how philosophers go about philosophizing and how they think about the role that LMs could play in substantively supporting their critical thinking.


% Philosophy, certainly since Plato declared that ``the unexamined life is not worth living'' and even earlier, has been concerned with critical thinking.
% Important philosophical questions -- e.g. X, Y, Z -- concern this basic move of systematically examining what something is.
% It's not just all about ``suspicion'', as Paul Ricoeur says, in which we discover what secretly has been living down here all along.
% There's also a way of reading things which ``recovers'' models, which attempts to breath live into them.
% Philosophy is ``the endeavour to know how and to what extent it might be possible to think differently, instead of legitimating what is already known?'' -- Michel Foucault


% We set out three.
% Plato said, ``the unexamined life is not worth living'' -- critical thinking involves subjecting all parts of our living to analysis.
% Decartes emphasized doubt -- we should not take things at their face value, but probe deeper.
% Ricoeur -- critical thinking is not merely about \textit{suspicion}, but also \textit{recovery}.
% Philosophy is the critical work that thought brings to bear on itself. -- Foucault

% What are the specific aims that modern professional philosophers set out for themselves? ...

% Every discipline does a little bit of philosophizing

% Bring in Rose's comment here about philosophers always engaging in the world

% Various features of philosophy

% Philosophy is not determined or easily verified
% Philosophy is very particular about language and concepts
% Philosophy challenges common-sense notions (uncommon sense?)

% There have been some works training LMs on philosophy, but the focus of this work is not particularly on helping philosophers.

% Philosophy has its fingers everywhere – there are few disciplines with as much cross-disciplinary potential, and philosophy can give you a foot in all of these areas, you can have real conversations with people working in these fields. (Garret)
% Language models already have a reasonable place to go.
% In some basic ways, LMs can start doing philosophy in the same way that humans can: by figuring out how to question the common sense which they seem to be improving upon.
% Since LMs have a substantive foothold on common sense, they're already one foot in the door.
% Cite some more metaphilosophical papers which talk about this -- in some sense you can take any X and do a 'philosophy of X' just by trying to clarify it and ask `why' questions down the wazoo...
% This is not true for other advanced areas of reasoning; mathematics and biology have clear and limited purviews of content, in addition to certain methodologies and features of their mode of inquiry.
% Even though solving advanced mathematics problems might require overlapping critical reasoning and creative skills, the language of mathematics is not one which current LMs are well-versed in currently, and training them requires special approaches \andre{maybe cite alpha geometry paper}
% \andre{add the following:}
% Indeed, the impression that philosophy is done in the armchair has always been a retroactive fantasy: there has been a rich tradition of philosophers which have engaged with the world. 
% Philosophy always was this attempt.
% \andre{Rose: there’s a point to be made here about how the best philosophy has always been in dialogue with the cutting edge intellectual inquiry of its time. Plato was drawing on advanced mathematics; Aristotle did extensive empirical work; Descartes was a physicist and mathematician; Hume’s work straddles the border between philosophy and empirical psychology; Hobbes is as much a political scientist as a philosopher; etc. etc. etc. The “armchair” conception of philosophers is in significant part a consequence of particular idiosyncrasies of the contemporary university; what that conception is responding to is not a distinguishing characteristic of philosophy as such.}


% Everyone does a little bit of philosophizing

% There is another reason why doing philosophy might be a productive focus for LMs in critical thinking: the text is the product.
% \textit{Text and language is fairly fundamental to doing philosophy.}
% The dominant mode of participation in philosophy is through texts and language.
% \icite{Garret} notes that philosophy doesn't do as much visual stuff as other disciplines like science.
% Certainly, philosophers suggest that there is more to the thinking and philosophizing than just what is written down, but the final article of professional philosophy often \textit{is} the article.
% On the other hand in the sciences, the natural language reports on the real object, which is the experiment.
% The genuine article of philosophy is already in text.
% This simplifies a lot of things for us.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

